Symbolic, numeric and quantum computation of Hartree-Fock equation

In this article, we discuss how a kind of hybrid computation, which employs symbolic, numeric, classic, and quantum algorithms, allows us to conduct Hartree-Fock electronic structure computation of molecules. In the proposed algorithm, we replace the Hartree-Fock equations with a set of equations composed of multivariate polynomials. We transform those polynomials to the corresponding Gr\"obner bases, and then we investigate the corresponding quotient ring, wherein the orbital energies, the LCAO coefficients, or the atomic coordinates are represented by the variables in the ring. In this quotient ring, the variables generate the transformation matrices that represent the multiplication with the monomial bases, and the eigenvalues of those matrices compose the roots of the equation. The quantum phase estimation (QPE) algorithm enables us to record those roots in the quantum states, which would be used in the input data for more advanced and more accurate quantum computations.

==> FABLEpy.tex <==
#!/usr/bin/env python
# coding: utf-8

# In[2]:


import numpy as np
from scipy.linalg import expm, sinm, cosm,logm
import scipy


# In[ ]:


#
# Transformation matrices.
#


# In[3]:


#
# V1(x,y)=V2(x,y)=0
#
mx=[
[0,   0,   0, -1],
[0,   0,   -1,0],
[0,   -1/2,0, 0],
[-1/2,0,   0, 0]]
my=[
[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[
[0,1,0,0],
[1,0,0,0],
[0,0,0,1],
[0,0,1,0]]


# In[4]:


import numpy as np
ee,vv=np.linalg.eig(np.array(me).transpose())
ww=vv.transpose()
print(ee)


# In[7]:


#
#  Prepare the eigenvectors of mx. 
#
v1=ww[1]
v2=ww[3]
vs=[v1,v2]
vs2=[0.57735027*v1+ 0.81649658*v2,0.57735027*v1- 0.81649658*v2]


# In[6]:


X=np.zeros((2,2))
for i in range(2):
    for j in range(2):
        X[i][j]=np.dot(vs[i],np.dot(np.array(mx).transpose(),vs[j]))
print(X)
print(np.linalg.eig(X))


# In[8]:


for t in vs2:
    a=np.dot(t,np.dot(np.array(mx).transpose(),t))
    b=np.dot(t,t)
    print(a/b)


# In[9]:


import pandas as pd
for mop in [mx,my,me]:
    print("m="+pd.DataFrame(mop).to_latex())


# In[79]:


#
# V1(x,y)=x*x,V2(x,y)=y*y
#
mx=[
[0,   0,   0, -2/3],
[0,   0,   -3/2,0],
[0,   -1/3,0, 0],
[-3/4,0,   0, 0]]
my=[
[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[
[0,1,0,0],
[9/4,0,0,0],
[0,0,0,1],
[0,0,9/4,0]]



# In[80]:


mx=[
[0,   0,   0, -1],
[0,   0,   -1,0],
[0,   -1/2,0, 0],
[-1/2,0,   0, 0]]
my=[
[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[
[0,1,0,0],
[1,0,0,0],
[0,0,0,1],
[0,0,1,0]]


# In[81]:


#
# V1(x,y)=V2(x,y)=(x-y)**2
#
mx=[[0,   0,   -1/2,-1/2],
[0,   0,   -3/2,1/2],
[-1/4,-1/4,0,   0],
[-3/4,1/4, 0,   0]]
my=[[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[[2,1,0,0],
[3,0,0,0],
[0,0,2,1],
[0,0,3,0]]
#e2-2e-3,
#8y2+e2-2e-7,
#2x+ye-y


# In[11]:


#
# V1(x,y)=V2(x,y)=(x-y)**2
#
mx=[[0,   0,   -1/2,-1/2],
[0,   0,   -3/2,1/2],
[-1/4,-1/4,0,   0],
[-3/4,1/4, 0,   0]]
my=[[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[[2,1,0,0],
[3,0,0,0],
[0,0,2,1],
[0,0,3,0]]
#e2-2e-3,
#8y2+e2-2e-7,
#2x+ye-y




# In[12]:


EXPMT=[expm(-1j*np.array(x)) for x in [mx,my,me]]


# In[13]:


eige,vece=np.linalg.eig(me)
eigx,vecx=np.linalg.eig(mx)
eigy,vecy=np.linalg.eig(my)


# In[14]:


eige


# In[15]:


vece


# In[18]:


eigy


# In[17]:


vecy


# In[89]:


eigx


# In[90]:


vecx


# In[19]:


l1=[0,2]
l2=[1,3]
for mop in [me,mx,my]:
    print("\n")
    A=np.zeros((2,2))
    B=np.zeros((2,2))
    for i in range(2):
        for j in range(2):
            ip=l1[i]
            jp=l1[j]
            A[i,j]=np.dot(vecy.transpose()[ip],np.dot(mop,vecy.transpose()[jp]))
            B[i,j]=np.dot(vecy.transpose()[ip],vecy.transpose()[jp])

    #print(A)
    #print(B)
    s,t=scipy.linalg.eig(A,B)
    print(s)
    print(t)


# In[20]:


l1=[0,2]
l2=[1,3]
for mop in [me,mx,my]:
    print("\n")
    A=np.zeros((2,2))
    B=np.zeros((2,2))
    for i in range(2):
        for j in range(2):
            ip=l2[i]
            jp=l2[j]
            A[i,j]=np.dot(vecx.transpose()[ip],np.dot(mop,vecx.transpose()[jp]))
            B[i,j]=np.dot(vecx.transpose()[ip],vecx.transpose()[jp])

    print(A)
    print(B)
    s,t=scipy.linalg.eig(A,B)
    print(s)
    print(t)


# In[21]:


#
#  Block Encoding
#
from fable import fable
from qiskit_aer import AerSimulator
import numpy as np


# In[22]:


def test_fable_real():
    n = 3
    a = np.random.randn(2**n, 2**n)++ 1j * np.random.randn(2**n, 2**n)

    simulator = AerSimulator(method="unitary")

    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  np.real(u_be[:2**n, :2**n])
    )


def test_fable_complex():
    n = 3
    a = np.random.randn(2**n, 2**n) + 1j * np.random.randn(2**n, 2**n)

    simulator = AerSimulator(method="unitary")

    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )


# In[23]:


EXPMT=[expm(-1j*np.array(x)) for x in [mx,my,me]]


# In[24]:


n = 2
a = np.random.randn(2**n, 2**n)+ 1j * np.random.randn(2**n, 2**n)
a = np.random.randn(2**n, 2**n) + 1j * np.random.randn(2**n, 2**n)
a=EXPMT[-1]
simulator = AerSimulator(method="unitary")

circ, alpha = fable(a)
circ.save_state()
u_be = simulator.run(circ).result().get_unitary().data
np.testing.assert_array_almost_equal(
    a/alpha/2**n,  u_be[:2**n, :2**n]
)


# In[25]:


print(a/alpha/2**n)
print(u_be[:2**n, :2**n])


# In[26]:


circ.draw("mpl")


# In[99]:


n = 2
#a=np.array([[1.,0,0,0],[0,1.,0,0],[0,0,1.,0],[0,0,0,1.]])
a=EXPMT[-1]
#a=np.array([[0,0.,0,1],[0.,0,0,0],[0,0,0,0],[1,0,0,0]])
simulator = AerSimulator(method="unitary")

circ, alpha = fable(a)
circ.save_state()
u_be = simulator.run(circ).result().get_unitary().data
np.testing.assert_array_almost_equal(
    a/alpha/2**n,  u_be[:2**n, :2**n]
)


# In[100]:


ee,vv=scipy.linalg.eig(np.array(me).transpose())
ww=vv.transpose()
print(ee)
print(ww)


# In[101]:


print(np.array(me))


# In[29]:


#
#  Test of Block Encoding of a simple toy model.
#
def stv(e,x,y):
#
#  The common eigenvecor
#
    n=2
    b=np.zeros(2**n)
    b[0]=y*e
    b[1]=y 
    b[2]=e
    b[3]=1
    return b

#
# e=-1
#
b=(stv(-1,1/np.sqrt(2),1/np.sqrt(2)))
print(b/np.sqrt(2))
print(np.dot(np.array(me).transpose(),b))
b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))

b=stv(3,1/np.sqrt(2),-1/np.sqrt(2))
print(b)
print(np.dot(np.array(me).transpose(),b))


# In[31]:


#
# V1(x,y)=V2(x,y)=0
#
mx=[
[0,   0,   0, -1],
[0,   0,   -1,0],
[0,   -1/2,0, 0],
[-1/2,0,   0, 0]]
my=[
[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[
[0,1,0,0],
[1,0,0,0],
[0,0,0,1],
[0,0,1,0]]

def stv(e,x,y):
    n=2
    b=np.zeros(2**n)
    b[0]=y*e
    b[1]=y 
    b[2]=e
    b[3]=1
    return b

#
# e=-1
#
lall=list()
b=(stv(-1,1/np.sqrt(2),1/np.sqrt(2)))
print(b)
liste1=list()
for mop in [mx,my,me]:
    mop=np.array(mop).transpose()
    mope=expm(-1j*np.array(mop))
    print(np.dot(mop,b))
    liste1.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
    lall.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))

#
# e=3
#
print("\n")
liste2=list()
b=stv(1,1/np.sqrt(2),-1/np.sqrt(2))
print(b)
for mop in [mx,my,me]:
    mop=np.array(mop).transpose()
    print(np.dot(mop,b))
    mope=expm(-1j*np.array(mop))
    liste2.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
    lall.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
#print(b)
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(-3j))


# In[104]:


import pandas as pd
pd1=pd.DataFrame(liste1,columns=["$Eig$","$\exp(-iEig)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
print(pd1.to_latex())


# In[105]:


pd2=pd.DataFrame(liste2,columns=["$Eig$","$\exp(-iEig)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
print(pd2.to_latex())


# In[32]:


pdall=pd.DataFrame(lall,columns=["$Eig$","$\exp(-iEig)$","$(\phi|O_A|\phi)$"],index=["mx","my","me","mx","my","me"])
print(pdall.to_latex())


# In[33]:


#
# V1(x,y)=V2(x,y)=(x-y)**2
#
mx=[[0,   0,   -1/2,-1/2],
[0,   0,   -3/2,1/2],
[-1/4,-1/4,0,   0],
[-3/4,1/4, 0,   0]]
my=[[0,  0,  1,0],
[0,  0,  0,1],
[1/2,0,  0,0],
[0,  1/2,0,0]]
me=[[2,1,0,0],
[3,0,0,0],
[0,0,2,1],
[0,0,3,0]]
#e2-2e-3,
#8y2+e2-2e-7,
#2x+ye-y


# In[109]:


def stv(e,x,y):
    n=2
    b=np.zeros(2**n)
    b[0]=y*e
    b[1]=y 
    b[2]=e
    b[3]=1
    return b

#
# e=-1
#
b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
print(b)
liste1=list()
for mop in [mx,my,me]:
    mop=np.array(mop).transpose()
    mope=expm(-1j*np.array(mop))
    print(np.dot(mop,b))
    liste1.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))

#
# e=3
#
print("\n")
liste2=list()
b=stv(3,1/np.sqrt(2),-1/np.sqrt(2))
print(b)
for mop in [mx,my,me]:
    mop=np.array(mop).transpose()
    print(np.dot(mop,b))
    mope=expm(-1j*np.array(mop))
    liste2.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope,b))/np.dot(b,b)])
#print(b)
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(-3j))


# In[110]:


import pandas as pd
pd1=pd.DataFrame(liste1,columns=["$E$","$\exp(-iE)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
pd1


# In[111]:


pd2=pd.DataFrame(liste2,columns=["$E$","$\exp(-iE)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
pd2


# In[112]:


circ.measure_all()


# In[113]:


circ.draw("mpl")


# In[114]:


from qiskit import Aer, transpile
from qiskit.tools.visualization import plot_histogram, plot_state_city
simulator = Aer.get_backend('aer_simulator')
circ = transpile(circ, simulator)


# In[115]:


result = simulator.run(circ,shots=100000).result()
counts = result.get_counts(circ)
plot_histogram(counts, title='Bell-State counts')


# In[116]:


simulator.run(circ).result()


# In[117]:


circ.draw("mpl")


# In[118]:


import numpy as np
from qiskit import QuantumCircuit


def gray_code(b):
    '''Gray code of b.
    Args:
        b: int:
            binary integer
    Returns:
        Gray code of b.
    '''
    return b ^ (b >> 1)


def gray_permutation(a):
    '''Permute the vector a from binary to Gray code order.

    Args:
        a: vector
            1D NumPy array of size 2**n
    Returns:
        vector:
            Gray code permutation of a
    '''
    b = np.zeros(a.shape[0])
    for i in range(a.shape[0]):
        b[i] = a[gray_code(i)]
    return b


def sfwht(a):
    '''Scaled Fast Walsh-Hadamard transform of input vector a.

    Args:
        a: vector
            1D NumPy array of size 2**n.
    Returns:
        vector:
            Scaled Walsh-Hadamard transform of a.
    '''
    n = int(np.log2(a.shape[0]))
    for h in range(n):
        for i in range(0, a.shape[0], 2**(h+1)):
            for j in range(i, i+2**h):
                x = a[j]
                y = a[j + 2**h]
                a[j] = (x + y) / 2
                a[j + 2**h] = (x - y) / 2
    return a


def compute_control(i, n):
    '''Compute the control qubit index based on the index i and size n.'''
    if i == 4**n:
        return 1
    return 2*n - int(np.log2(gray_code(i-1) ^ gray_code(i)))


def compressed_uniform_rotation(a, ry=True):
    '''Compute a compressed uniform rotation circuit based on the thresholded
    vector a.

    Args:
        a: vector:
            A thresholded vector a a of dimension 2**n
        ry: bool
            uniform ry rotation if true, else uniform rz rotation
    Returns:
        circuit
            A qiskit circuit representing the compressed uniform rotation.
    '''
    n = int(np.log2(a.shape[0])/2)
    circ = QuantumCircuit(2*n + 1)

    i = 0
    while i < a.shape[0]:
        parity_check = 0

        # add the rotation gate
        if a[i] != 0:
            if ry:
                circ.ry(a[i], 0)
            else:
                circ.rz(a[i], 0)

        # loop over sequence of consecutive zeros
        while True:
            ctrl = compute_control(i+1, n)
            # toggle control bit
            parity_check = (parity_check ^ (1 << (ctrl-1)))
            i += 1
            if i >= a.shape[0] or a[i] != 0:
                break

        # add CNOT gates
        for j in range(1, 2*n+1):
            if parity_check & (1 << (j-1)):
                circ.cnot(j, 0)

    return circ


# In[119]:


def fable(a, epsilon=None):
    '''FABLE - Fast Approximate BLock Encodings.

    Args:
        a: array
            matrix to be block encoded.
        epsilon: float >= 0
            (optional) compression threshold.
    Returns:
        circuit: qiskit circuit
            circuit that block encodes A
        alpha: float
            subnormalization factor
    '''
    epsm = np.finfo(a.dtype).eps
    alpha = np.linalg.norm(np.ravel(a), np.inf)
    if alpha > 1:
        alpha = alpha + np.sqrt(epsm)
        a = a/alpha
    else:
        alpha = 1.0

    n, m = a.shape
    if n != m:
        k = max(n, m)
        a = np.pad(a, ((0, k - n), (0, k - m)))
        n = k
    logn = int(np.ceil(np.log2(n)))
    if n < 2**logn:
        a = np.pad(a, ((0, 2**logn - n), (0, 2**logn - n)))
        n = 2**logn

    a = np.ravel(a)
    #print("a",a)
    if all(np.abs(np.imag(a)) < epsm):  # real data
        a = gray_permutation(
                sfwht(
                    2.0 * np.arccos(np.real(a))
                )
            )
        # threshold the vector
        #print(a)
        if epsilon:
            a[abs(a) <= epsilon] = 0
        # compute circuit
        OA = compressed_uniform_rotation(a)
    else:  # complex data
        # magnitude
        a_m = gray_permutation(
                sfwht(
                    2.0 * np.arccos(np.abs(a))
                )
            )
        if epsilon:
            a_m[abs(a_m) <= epsilon] = 0

        # phase
        a_p = gray_permutation(
                sfwht(
                    -2.0 * np.angle(a)
                )
            )
        if epsilon:
            a_p[abs(a_p) <= epsilon] = 0

        # compute circuit
        OA = compressed_uniform_rotation(a_m).compose(
                compressed_uniform_rotation(a_p, ry=False)
            )

    circ = QuantumCircuit(2*logn + 1)

    # diffusion on row indices
    for i in range(logn):
        circ.h(i+1)

    # matrix oracle
    circ = circ.compose(OA)

    # swap register
    for i in range(logn):
        circ.swap(i+1,  i+logn+1)

    # diffusion on row indices
    for i in range(logn):
        circ.h(i+1)

    # reverse bits because of little-endiannes
    circ = circ.reverse_bits()

    return circ, alpha

circ, alpha = fable(a)


# 
# 
# 

# # Hatree-Fock Computaion of a realistic molecule
# 
# 
# ```
# OBJ=281*R**5*x**3*y + 1119*R**5*x**2*y**2 + 164*R**5*x**2 + 533*R**5*x*y**3 - 901*R**5*x*y - 70*R**5*y**2 - 1756*R**5 - 2892*R**4*x**3*y - 9431*R**4*x**2*y**2 - 2273*R**4*x**2 - 5040*R**4*x*y**3 + 8552*R**4*x*y + 712*R**4*y**2 + 15802*R**4 + 11305*R**3*x**3*y + 29175*R**3*x**2*y**2 + 12477*R**3*x**2 + 18393*R**3*x*y**3 - 30849*R**3*x*y - 1877*R**3*y**2 - 59260*R**3 - 15964*R**2*x**3*y - 32038*R**2*x**2*y**2 - 35996*R**2*x**2 - 27890*R**2*x*y**3 + 37012*R**2*x*y - 3516*R**2*y**2 + 118518*R**2 - 12479*R*x**3*y - 18807*R*x**2*y**2 + 58692*R*x**2 + 1281*R*x*y**3 + 52833*R*x*y + 28135*R*y**2 - 133334*R - 2*e*(114*R**5*x*y - 1281*R**4*x*y + 5600*R**3*x*y - 10194*R**2*x*y + 115*R*x*y + 10000*x**2 + 18221*x*y + 10000*y**2 - 10000) + 13071*x**4 + 45874*x**3*y + 59634*x**2*y**2 - 91649*x**2 + 32206*x*y**3 - 146963*x*y + 7746*y**4 - 65195*y**2 + 79999;
# ```
# 
# 
# 

# In[34]:


import numpy as np
import csv
def getmat(filename):
    rowmx=list()
    with open(filename, 'r') as file:
        reader = csv.reader(file)
        for t in reader:
            #print(t)
            rowmx.append(t)
    x=rowmx[0]
    y=np.array([eval(t) for t in x])
    return np.array(np.array_split(y,8))

mx=getmat('save_mx.txt')    
my=getmat('save_my.txt')    
me=getmat('save_me.txt')   

mx=mx.transpose()
my=my.transpose()
me=me.transpose()


# In[35]:


#
# Check the block-encoding. !No problem.
#
simulator = AerSimulator(method="unitary")
circlist=list()
for a in [mx,my,me]:
    n=3
    a=expm(-1j*a)
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    circlist.append(u_be)
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    #print(alpha*2**n*np.real(np.dot(www.conj(),np.dot(u_be[:2**n, :2**n],www))))
    #print(np.exp(-1j*alpha*2**n*np.real(np.dot(www.conj(),np.dot(u_be[:2**n, :2**n],www)))))


# In[37]:


#
# e=-1
#
emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]

liste1=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=np.array(mop)
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste1.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.dot(b,np.dot(mop,b))/np.dot(b,b),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1

b=vmy[-2]
liste2=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=np.array(mop)
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste2.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.dot(b,np.dot(mop,b))/np.dot(b,b),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:


# In[38]:


import pandas as pd
pd.options.display.precision = 6
pd1=pd.DataFrame(liste1,columns=["$E$","$(\phi|A|\phi)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
print(emy[-1])
pd1


# In[39]:


SZABOE="                           1                  2\
         1       -0.1597448132D+01   0.0000000000D+00\
         2        0.0000000000D+00  -0.6166851652D-01"
SZABOXY="                          1                  2\
         1        0.8019175078D+00  -0.7822652261D+00\
         2        0.3368004878D+00   0.1068445602D+01"


# In[40]:


SZABOCALC=[SZABOXY.split()[3].replace("D","e"),SZABOXY.split()[6].replace("D","e"),SZABOE.split()[3].replace("D","e")]
SZABOCALC=[[float(x) for x in SZABOCALC]]
import pandas as pd
pd.options.display.precision =6
pdSZABO=pd.DataFrame(SZABOCALC,columns=["$e$","$x$","$y$"],index=["STO-3G"])
print(pdSZABO.to_latex())


# In[41]:


import pandas as pd
pd.options.display.precision = 6
pd2=pd.DataFrame(liste1,columns=["$E$","$(\phi|A|\phi)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
print(emy[-2])
pd2


# In[42]:


#
# e=-1
#
emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]
liste1=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=expm(-1j*np.array(mop))
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste1.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1

b=vmy[-2]
liste2=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=expm(-1j*np.array(mop))
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste2.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste2


# In[43]:


#
# e=-1
#
emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]
liste1=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=expm(-1j*np.array(mop))
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste1.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1

b=vmy[-2]
liste2=list()
for mop in [mx,my,me]:
    mop=np.array(mop)
    mope=expm(-1j*np.array(mop))
    #print(np.dot(mop,b))
    a=mope
    circ, alpha = fable(a)
    circ.save_state()
    u_be = simulator.run(circ).result().get_unitary().data
    np.testing.assert_array_almost_equal(
        a/alpha/2**n,  u_be[:2**n, :2**n]
    )
    mope2=alpha*2**n*u_be[:2**n, :2**n]
    liste2.append([np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
         np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste2


# In[44]:


import pandas as pd
pd.options.display.precision = 6
pd1=pd.DataFrame(liste1,columns=["$E$","$\exp(-iE)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
pd1


# In[45]:


import pandas as pd
pd2=pd.DataFrame(liste1,columns=["$E$","$\exp(-iE)$","$(\phi|O_A|\phi)$"],index=["mx","my","me"])
pd2


# In[46]:


emx, wmx=np.linalg.eig(mx)
eme, wme=np.linalg.eig(me)


# In[47]:


emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]


listeC=list()
id=0
for e,b in zip(emy,vmy):
    locallist=list()
    if np.abs(np.imag(e))<1.0e-10:
        id+=1  
        locallist.append(e)   
        for mop ,mtype in zip([mx,my,me],["$m_x$","$m_y$","$m_e$"]):
            mop=np.array(mop)
            mope=np.array(mop)
            locallist.append(np.dot(b,np.dot(mop,b))/np.dot(b,b))
        listeC.append(locallist)
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1
listeC


# In[48]:


listeC
import pandas as pd
pd.options.display.precision = 6
pdC=pd.DataFrame(listeC,columns=["$\text{Eig}$","$(\phi|m_x^T|\phi)$","$(\phi|m_y^T|\phi)$","$(\phi|m_e^T|\phi)$"])
print(emy[-2])
print(pdC.to_latex())


# In[49]:


emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]


listeB=list()
id=0
for e,b in zip(emy,vmy):
    if np.abs(np.imag(e))<1.0e-10:
        id+=1  
        for mop ,mtype in zip([mx,my,me],["$m_x$","$m_y$","$m_e$"]):
            mop=np.array(mop)
            mope=np.array(mop)
            #print(np.dot(mop,b))
            a=mope
            circ, alpha = fable(a)
            circ.save_state()
            u_be = simulator.run(circ).result().get_unitary().data
            np.testing.assert_array_almost_equal(
                a/alpha/2**n,  u_be[:2**n, :2**n]
            )
            mope2=alpha*2**n*u_be[:2**n, :2**n]
            listeB.append([mtype,np.dot(b,np.dot(mop,b))/np.dot(b,b),np.dot(b,np.dot(mop,b))/np.dot(b,b),\
                 np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
  
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1


# In[50]:


listeB
import pandas as pd
pd.options.display.precision = 6
pdB=pd.DataFrame(listeB,columns=["$M$","$\text{Eig}$","$(\phi|M|\phi)$","$(\phi|O_M|\phi)$"],\
                 index=["1","1","1","2","2","2","3","3","3","3","3","3"])
print(emy[-2])
pdB


# In[51]:


emy, wmy=np.linalg.eig(my)
vmy=wmy.transpose()
print(emy)
#b=(stv(-1,1/np.sqrt(2),-1/np.sqrt(2)))
b=vmy[-2]


listeA=list()
id=0
for e,b in zip(emy,vmy):
    if np.abs(np.imag(e))<1.0e-10:
        id+=1  
        for mop ,mtype in zip([mx,my,me],["$m_x$","$m_y$","$m_e$"]):
            mop=np.array(mop)
            mope=expm(-1j*np.array(mop))
            #print(np.dot(mop,b))
            a=mope
            circ, alpha = fable(a)
            circ.save_state()
            u_be = simulator.run(circ).result().get_unitary().data
            np.testing.assert_array_almost_equal(
                a/alpha/2**n,  u_be[:2**n, :2**n]
            )
            mope2=alpha*2**n*u_be[:2**n, :2**n]
            listeA.append([mtype,np.dot(b,np.dot(mop,b))/np.dot(b,b),np.exp(-1j*np.dot(b,np.dot(mop,b))/np.dot(b,b)),\
                 np.dot(b,np.dot(mope2,b))/np.dot(b,b)])
  
#for mop in EXPMT:
#    print(np.dot(b,np.dot(mop,b))/np.dot(b,b))
#bb=2**n*alpha*np.dot(u_be[:2**n, :2**n],b)
#print(bb[3],np.exp(1j))
#liste1



# In[52]:


listeA
import pandas as pd
pd.options.display.precision = 6
pdA=pd.DataFrame(listeA,columns=["$M$","$\text{Eig}$","$(\phi|\exp(-\sqrt{-1}M)|\phi)$","$(\phi|O_{\exp}|\phi)$"],\
                 index=["1","1","1","2","2","2","3","3","3","4","4","4"])
print(emy[-2])
print(pdA.to_latex())



==> SCRIPT.tex <==
This file contains the Singular script used in the study
"Symbolyc-numeric and classic-quantum hybrid computation of Hartree-Fock equations" by Ichio Kikuchi, Akihito Kikuchi


(1) The script defines the ring Q[x,y,e,R] 
where
 (x,y) : the wave function
 e     : orbital energy
 R     : The bond length
 with degree reverse lexicographic monomial ordering.

(2) It generates the polynomial ideal (I) from the objective function OBJ. 

(3) It computes the standard basis (SI) of the ideal I.

(4) It transforms (SI) to the standard basis (j) in the lexicographic monomial ordering. 

(5) It solves the system of polynomial equations by the triangulation. 

(6) It generates the transformation matrices (mx,my,me,mr) 
for x, y, e, R in Q[x,y,e,R]/I and write them in text files. 

----(Singular Script)---------------------------------------

LIB "solve.lib";option(redSB);
ring r1=0,(x,y,e,R),dp;
poly OBJ=281*R**5*x**3*y + 1119*R**5*x**2*y**2 + 164*R**5*x**2 + 533*R**5*x*y**3 - 901*R**5*x*y - 70*R**5*y**2 - 1756*R**5 - 2892*R**4*x**3*y - 9431*R**4*x**2*y**2 - 2273*R**4*x**2 - 5040*R**4*x*y**3 + 8552*R**4*x*y + 712*R**4*y**2 + 15802*R**4 + 11305*R**3*x**3*y + 29175*R**3*x**2*y**2 + 12477*R**3*x**2 + 18393*R**3*x*y**3 - 30849*R**3*x*y - 1877*R**3*y**2 - 59260*R**3 - 15964*R**2*x**3*y - 32038*R**2*x**2*y**2 - 35996*R**2*x**2 - 27890*R**2*x*y**3 + 37012*R**2*x*y - 3516*R**2*y**2 + 118518*R**2 - 12479*R*x**3*y - 18807*R*x**2*y**2 + 58692*R*x**2 + 1281*R*x*y**3 + 52833*R*x*y + 28135*R*y**2 - 133334*R - 2*e*(114*R**5*x*y - 1281*R**4*x*y + 5600*R**3*x*y - 10194*R**2*x*y + 115*R*x*y + 10000*x**2 + 18221*x*y + 10000*y**2 - 10000) + 13071*x**4 + 45874*x**3*y + 59634*x**2*y**2 - 91649*x**2 + 32206*x*y**3 - 146963*x*y + 7746*y**4 - 65195*y**2 + 79999;
list diffs;
for(int i=1;i<=nvars(r1); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}
poly fR=100*R-146;
ideal I=fR;
for(int i=1;i<=nvars(r1)-1; i=i+1){I=I+diff(OBJ,var(i));}
ideal SI=std(I);
ring s=0,(x,y,e,R),lp;
setring s;
ideal j=fglm(r1,SI);
def R=triang_solve(j,10);
setring R;rlist;
setring r1;
LIB "rootsmr.lib";
ideal b=qbase(SI);
matrix mx=matmult(x,b,SI);
matrix my=matmult(y,b,SI);
matrix me=matmult(e,b,SI);
write(":w b.txt",string(b));
write(":w save_mx.txt",string(mx));
write(":w save_my.txt",string(my));
write(":w save_me.txt",string(me));


LIB "solve.lib";option(redSB);
ring r0=0,(x,y,e,R),dp;
poly OBJ=-216*R**6*x**3*y - 513*R**6*x**2*y**2 + 227*R**6*x**2 - 102*R**6*x*y**3 + 1189*R**6*x*y - 54*R**6*y**2 + 1170*R**6 + 2222*R**5*x**3*y + 5732*R**5*x**2*y**2 - 1885*R**5*x**2 + 1448*R**5*x*y**3 - 11608*R**5*x*y + 408*R**5*y**2 - 12291*R**5 - 10170*R**4*x**3*y - 26729*R**4*x**2*y**2 + 5413*R**4*x**2 - 8470*R**4*x*y**3 + 48703*R**4*x*y - 1082*R**4*y**2 + 55308*R**4 + 25861*R**3*x**3*y + 63770*R**3*x**2*y**2 - 2893*R**3*x**2 + 25252*R**3*x*y**3 - 111151*R**3*x*y + 1710*R**3*y**2 - 138272*R**3 - 32339*R**2*x**3*y - 70957*R**2*x**2*y**2 - 18704*R**2*x**2 - 35606*R**2*x*y**3 + 127352*R**2*x*y - 7552*R**2*y**2 + 207407*R**2 - 2654*R*x**3*y + 4544*R*x**2*y**2 + 48317*R*x**2 + 5911*R*x*y**3 - 1371*R*x*y + 30556*R*y**2 - 186667*R - 2*e*(-22*R**6*x*y + 310*R**5*x*y - 2014*R**4*x*y + 7068*R**3*x*y - 11845*R**2*x*y + 1106*R*x*y + 10000*x**2 + 17974*x*y + 10000*y**2 - 10000) + 13071*x**4 + 43417*x**3*y + 53796*x**2*y**2 - 89055*x**2 + 31049*x*y**3 - 133412*x*y + 7746*y**4 - 65800*y**2 + 93333;
list diffs;
for(int i=1;i<=nvars(r0); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}
poly fR=100*R-146;
ideal I=fR;
for(int i=1;i<=nvars(r0)-1; i=i+1){I=I+diff(OBJ,var(i));}
ideal SI=std(I);
ring s=0,(x,y,e,R),lp;
setring s;
ideal j=fglm(r0,SI);
def RS=triang_solve(j,10);
setring RS;rlist;
setring r0;
LIB "rootsmr.lib";
ideal b=qbase(SI);
matrix mx = matmult(x,b,SI);
matrix me = matmult(e,b,SI);
matrix my = matmult(y,b,SI);
write(":w save_mx.txt",string(mx));
write(":w save_my.txt",string(my));
write(":w save_me.txt",string(me));
write(":w save_qb.txt",string(b));

----(Singular Script)---------------------------------------


The matrix data are read and transformed to Python numpy arrays.

----(Python Script)---------------------------------------

import numpy as np
import csv
def getmat(filename):
    rowmx=list()
    with open(filename, 'r') as file:
        reader = csv.reader(file)
        for t in reader:
            #print(t)
            rowmx.append(t)
    x=rowmx[0]
    y=np.array([eval(t) for t in x])
    return np.array(np.array_split(y,8))

mx=getmat('save_mx.txt')    
my=getmat('save_my.txt')    
me=getmat('save_me.txt')    
mx=mx.transpose()
my=my.transpose()
me=me.transpose()

ee,ww=np.linalg.eig(mx)
vv=ww.transpose()

LE=list()
for v in vv:
    LE2=[np.dot(v.conj().transpose(),np.dot(A,v)) for A in [mx,my,me]]
    LE.append(LE2)
    
import pandas as pd
DFL=pd.DataFrame(LE,columns=["(i|mx|i)","(i|my|i)","(i|me|i)",])
print(DFL)

----(Python Script)---------------------------------------

==> SZ-SYM-RHF.tex <==
#!/usr/bin/env python
# coding: utf-8

# In[1]:


import sympy 
sympy.__version__
x, y, R= sympy.symbols("x y R")
expr=0.56*sympy.exp(1*R*R)
[expr.series(R,1.21233).removeO(),
expr.subs(R,1.46)]


# In[20]:


import sympy as sympy
from sympy import symbols, Function,expand,core,sqrt
import numpy as np

from sympy import symbols, Function,expand,sqrt
import numpy as np
import copy

S12,T11,T12,T22,V11A,V12A,V22A,V11B,V12B,V22B,V1111,V2111,V2121,V2211,V2221,V2222=[0 for _ in range(16)]
S=[[0 for _ in range(2)] for _ in range(2)]
X=[[0 for _ in range(2)] for _  in range(2)]
NM=[[0 for _ in range(2)] for _  in range(2)]
XT=[[0 for _ in range(2)] for _ in  range(2)]
H=[[0 for _ in range(2)] for _ in  range(2)]
F=[[0 for _ in range(2)] for _ in  range(2)]
G=[[0 for _ in range(2)] for _ in  range(2)]
C=[[0 for _ in range(2)] for _ in  range(2)]
FPRIME=[[0 for _ in range(2)] for _  in range(2)]
CPRIME=[[0 for _ in range(2)] for _  in range(2)]
P=[[0 for _ in range(2)] for _  in range(2)]
ODLPP=[[0 for _ in range(2)] for _  in range(2)]
E=[[0 for _ in range(2)] for _  in range(2)]
TT=[[[[0 for _ in range(2)] for _  in range(2)] for _ in range(2)] for _ in range(2)]


IOP=2
#
# CHOOSE STO-NG
#
N=3
R=1.4632
#
# Gaussian exponents:
# He:ZETA1; H;ZETA2
#
ZETA1=2.0925
ZETA2=1.24
#
#
#
ZA=2.0
ZB=1.0
#
# ATOMIC DISTANCE 
#
R=symbols("R",positive=True)
# WAVEFUNCTION (x,y)
x, y = symbols("x y")


def F0(ARG):
#
# F0 FUNCTION
#
    PI = np.pi
    if  type(ARG)==float and ARG < 1.0e-6:
        return 1 -ARG/3.
    if  type(ARG)==sympy.numbers.Zero and ARG < 1.0e-6:
        return 1 -ARG/3.
    else:
        #print("F0:ARG",ARG)
        return sqrt(PI/ARG)*sympy.erf(sqrt(ARG))/2
    
def getS(A,B,RAB2):
#
# Calculates the overlap matrix
#   
    PI=np.pi
    #print(A,B,RAB2)
    return (PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def getT(A,B,RAB2):
#
# Calculates the kinetic energy.
#
    PI=np.pi
    return A*B/(A+B)*(3.0-2.0*A*B*RAB2/(A+B))*(PI/(A+B))**1.5*sympy.exp(-A*B*RAB2/(A+B))

def V(A,B,RAB2,RCP2,ZC):
#
#  CALCULATES UN-NORMALIZED NUCLEAR ATTRACTION INTEGRALS
#
    PI=np.pi
    V=2.0*PI/(A+B)*F0((A+B)*RCP2)*sympy.exp(-A*B*RAB2/(A+B))
    return -V*ZC

def TWOE(A,B,C,D,RAB2,RCD2,RPQ2):
#
# CALCULATES TWO-ELECTRON INTEGRALS FOR UN-NORMALIZED PRIMITIVES
# A,B,C,D ARE THE EXPONENTS ALPHA, BETA, ETC.
# RAB2 EQUALS SQUARED DISTANCE BETWEEN CENTER A AND CENTER B, ETC.
#
    PI=np.pi
    return 2.0*(PI**2.5)/((A+B)*(C+D)*np.sqrt(A+B+C+D))*F0((A+B)*(C+D)*RPQ2/(A+B+C+D))*sympy.exp(-A*B*RAB2/(A+B)-C*D*RCD2/(C+D))

def INTGRL_SIMBOL(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
#  CALCULATES ALL THE BASIC INTEGRALS NEEDED FOR SCF CALCULATION
#
    global S12,T11,T12,T22,V11A,V12A,V22A,V11B,V12B,V22B,V1111,V2111,V2121,V2211,V2221,V2222
    COEF=[[1.0,0.0,0.0],[0.678914,0.430129,0.0],[0.444635,0.535328,0.154329]]
    EXPON=[[0.270950,0.0,0.0],[0.151623,0.851819,0.0],[0.109818,0.405771,2.22766]]
    R2=R*R
    N=3
    A1=[0 for I in range(N)]
    D1=[0 for I in range(N)]
    A2=[0 for I in range(N)]
    D2=[0 for I in range(N)]
    PI=np.pi

    for i in range(N):
        #print(i,EXPON[N-1][i],COEF[N-1][i],ZETA1,ZETA2)
        A1[i]=EXPON[N-1][i]*ZETA1**2
        D1[i]=COEF[N-1][i]*((2.0*A1[i]/PI)**0.75)
        A2[i]=EXPON[N-1][i]*(ZETA2**2)
        D2[i]=COEF[N-1][i]*((2.0*A2[i]/PI)**0.75)

    #print("A1",A1,"D1",D1,"A2",A2,"D2",D2)
        
    S12=0.0
    T11=0.0
    T12=0.0
    T22=0.0
    V11A=0.0
    V12A=0.0
    V22A=0.0
    V11B=0.0
    V12B=0.0
    V22B=0.0
    V1111=0.0
    V2111=0.0
    V2121=0.0
    V2211=0.0
    V2221=0.0
    V2222=0.0
    
    for I in range(N):
        for J in range(N):
            RAP=A2[J]*R/(A1[I]+A2[J])
            RAP2=RAP**2
            RBP2=(R-RAP)**2
            S12+=getS(A1[I],A2[J],R2)*D1[I]*D2[J]
            T11=T11+getT(A1[I],A1[J],0.0)*D1[I]*D1[J]
            #print(I,J,getT(A1[I],A1[J],0.0),D1[I],D1[J],T11)
            T12=T12+getT(A1[I],A2[J],R2)*D1[I]*D2[J]
            T22=T22+getT(A2[I],A2[J],0.0)*D2[I]*D2[J]
            V11A=V11A+V(A1[I],A1[J],0.0,0.0,ZA)*D1[I]*D1[J]
            V12A=V12A+V(A1[I],A2[J],R2,RAP2,ZA)*D1[I]*D2[J]
            V22A=V22A+V(A2[I],A2[J],0.0,R2,ZA)*D2[I]*D2[J]
            V11B=V11B+V(A1[I],A1[J],0.0,R2,ZB)*D1[I]*D1[J]
            V12B=V12B+V(A1[I],A2[J],R2,RBP2,ZB)*D1[I]*D2[J]
            V22B=V22B+V(A2[I],A2[J],0.0,0.0,ZB)*D2[I]*D2[J]
        
    for I in range(N):
        for J in range(N):
            for K in range(N):
                for L in range(N):
                    RAP=A2[I]*R/(A2[I]+A1[J])
                    RBP=R-RAP
                    RAQ=A2[K]*R/(A2[K]+A1[L])
                    RBQ=R-RAQ
                    RPQ=RAP-RAQ
                    RAP2=RAP*RAP
                    RBP2=RBP*RBP
                    RAQ2=RAQ*RAQ
                    RBQ2=RBQ*RBQ
                    RPQ2=RPQ*RPQ
                    V1111=V1111+TWOE(A1[I],A1[J],A1[K],A1[L],0.0,0.0,0.0)*D1[I]*D1[J]*D1[K]*D1[L]
                    V2111=V2111+TWOE(A2[I],A1[J],A1[K],A1[L],R2,0.0,RAP2)*D2[I]*D1[J]*D1[K]*D1[L]
                    V2121=V2121+TWOE(A2[I],A1[J],A2[K],A1[L],R2,R2,RPQ2)*D2[I]*D1[J]*D2[K]*D1[L]
                    V2211=V2211+TWOE(A2[I],A2[J],A1[K],A1[L],0.0,0.0,R2)*D2[I]*D2[J]*D1[K]*D1[L]
                    V2221=V2221+TWOE(A2[I],A2[J],A2[K],A1[L],0.0,R2,RBQ2)*D2[I]*D2[J]*D2[K]*D1[L]
                    V2222=V2222+TWOE(A2[I],A2[J],A2[K],A2[L],0.0,0.0,0.0)*D2[I]*D2[J]*D2[K]*D2[L]

    

def COLLECT(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# THIS TAKES THE BASIC INTEGRALS FROM COMMON AND ASSEMBLES THE
# RELEVENT MATRICES, THAT IS S,H,X,XT, AND TWO-ELECTRON INTEGRALS
#
    global H,S,X,TT,XT
    H[0][0]=T11+V11A+V11B
    H[0][1]=T12+V12A+V12B
    H[1][0]=H[0][1]
    H[1][1]=T22+V22A+V22B

    S[0][0]=1.
    S[0][1]=S12
    S[1][0]=S[0][1]
    S[1][1]=1.


    TT[0][0][0][0]=V1111
    TT[1][0][0][0]=V2111
    TT[0][1][0][0]=V2111
    TT[0][0][1][0]=V2111
    TT[0][0][0][1]=V2111
    TT[1][0][1][0]=V2121
    TT[0][1][1][0]=V2121
    TT[1][0][0][1]=V2121
    TT[0][1][0][1]=V2121
    TT[1][1][0][0]=V2211
    TT[0][0][1][1]=V2211
    TT[1][1][1][0]=V2221
    TT[1][1][0][1]=V2221
    TT[1][0][1][1]=V2221
    TT[0][1][1][1]=V2221
    TT[1][1][1][1]=V2222


    return

def MATOUT(A,IM,IN,M,N,LABEL):
    print(LABEL)
    print(A)
    return

def MULT(A,B,C,IM,M):
    for i in range(2):
        for j in range(2):
            C[i][j]=0
            for k in range(2):
                C[i][j]+=A[i][k]*B[k][j]
    return 

def FORMG():
#
# Calculates G matrix from density matrix and two-electron integrals
#
    global G,P,TT
    for I in range(2):
        for J in range(2):
            G[I][J]=0
            for K in range(2):
                for L in range(2):
                    #print(I,J,K,L,P[K][L],TT[I][J][K][L],TT[I][L][J][K],G[I][J])
                    G[I][J]+=P[K][L]*(TT[I][J][K][L]-0.5*TT[I][L][J][K])
    #print("G",G)
    return 



def SCF_SIMBOL(IOP,N,R,ZETA1,ZETA2,ZA,ZB):
#
# PREPARES THE ANALYTIC FORMULA OF THE TOTAL ENERGY.
#
    global G,C,FPRIME,CPRIME

    PI=np.pi
    CRIT=1.0e-4
    MAXIT=25
    ITER=0
    for I in range(2):
        for J in range(2):
            P[I][J]=0.
    P[0][0]=x*x*2
    P[0][1]=x*y*2
    P[1][0]=x*y*2
    P[1][1]=y*y*2
    
    MAXIT=1
    for ITER in range(MAXIT):
        
        FORMG()
        for i in range(2):
            for j in range(2):
                F[i][j]=H[i][j]+G[i][j]
        EN=0
        for i in range(2):
            for j in range(2):
                EN+=0.5*P[i][j]*(H[i][j]+F[i][j])

    ENT=EN+ZA*ZB/R

    return EN,ENT

#
# COMPUTES THE ELECTRON ENERGY (EN) and THE TOTAL ENERGY(ENT)
#
INTGRL_SIMBOL(IOP,N,R,ZETA1,ZETA2,ZA,ZB)
COLLECT(IOP,N,R,ZETA1,ZETA2,ZA,ZB)
EN,ENT=SCF_SIMBOL(IOP,N,R,ZETA1,ZETA2,ZA,ZB)

from sympy import Symbol, cos, series

#
print("CHECK THE TOTAL ENERGY: BY THIS SUBSTITUTION WE'LL GET THE VALUE CLOSE TO -2.86...")
#
print(ENT.subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)]))

# TAYLOR EXPANSION OF THE TOTAL ENERGY AROUNR R0=1.5
ENTS=series(expand(ENT),R,1.5)
ENTS2=expand(ENTS.removeO())
print("CHECK THE TOTAL ENERGY: BY THIS SUBSTITUTION WE'LL GET THE VALUE CLOSE TO -2.86...")
print(sympy.N(ENTS2.subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)])))

#
# THE NORMALIZARION CONDITION OF THE WAVE FUNCTION
#
W=[0,0]
W[0]=S[0][0]*x+S[0][1]*y
W[1]=S[1][0]*x+S[1][1]*y
NORMC=expand(x*W[0]+y*W[1])

#
# THE NORMALIZATION CONDITION AFTER TAYLOR EXPANSION
#
NORMCS=expand(series(NORMC,R,1.5).removeO())
print("CHECK THE NOTMALIZATION: BY THIS SUBSTITUTION WE'LL GET THE VALUE CLOSE TO 1...")
print(NORMCS.subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)]))

#
# TURN THE POLYNOMIAL ENERGY FUNCTIONAL INTO A SYMPY-POLYNOMIAL
#
ENTS3=sympy.poly(sympy.N(ENTS2))

#
# GET THE OBJECTIVE FUNTION WITH INTEGER COEFFICIENTS
#

def getINT(x,N):
#
#  ROWND DOWN x*N AFTER THE DECIMAL POINT and get AN INTEGER M
#  THEN X is approximated by M/N. 
#
    return (int(np.floor(x*N)))

AT=ENTS3.terms()
getF=0
for tm in AT:
    p0,p1,p2=tm[0]
    cf=tm[1]
    #print(p0,p1,p2,cf)
    getF+=x**p0*y**p1*R**p2*getINT(cf,10000)

AT=sympy.poly(NORMCS-1).terms()
getNS=0
for tm in AT:
    p0,p1,p2=tm[0]
    cf=tm[1]
    #print(p0,p1,p2,cf)
    getNS+=x**p0*y**p1*R**p2*getINT(cf,10000)

print((NORMCS-1).subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)]))
print(ENTS3.subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)]))
print(getNS.subs([(x,-0.80191751),(y,-0.33680049),(R,1.463)]))

e=symbols("e")

#
# GET THE OBJECTIVE FUNCTION
#
OF=getF-2*e*getNS

#
# PREPARES A Singular SCRIPT. 
#
#  If you are a user of Singular, you simply do as follows.
#
#  >> Singular < SCRIPT.txt
#
stringQ='LIB "solve.lib";option(redSB);\n'
stringQ+='ring r1=0,(x,y,e,R),dp;\n'+'poly OBJ='+str(OF)+';\n'
stringQ+='list diffs;\n'
stringQ+='for(int i=1;i<=nvars(r1); i=i+1){diffs=insert(diffs,diff(OBJ,var(i)));}\n'
stringQ+='poly fR=100*R-146;\n'
stringQ+='ideal I=fR;\n'
stringQ+='for(int i=1;i<=nvars(r1)-1; i=i+1){I=I+diff(OBJ,var(i));}\n'
stringQ+='ideal SI=std(I);\n'
stringQ+='ring s=0,(x,y,e,R),lp;\n'
stringQ+='setring s;\n'
stringQ+='ideal j=fglm(r1,SI);\n'
stringQ+='def R=triang_solve(j,10);\n'
stringQ+='setring R;rlist;'


text_file = open("SCRIPT.txt", "w")
 
#write string to file
on = text_file.write(stringQ)
 
#close file
text_file.close()

stringQ

#
# GET THE DIFFERENTIALS OF THE OBJECTIVE FUNCTION.
#
DS=[]
for t in [x,y,e,R]:
    DS.append(sympy.diff(OF,t))
index=0
for i in DS:
    print("poly f"+str(index)+"=",i,";")
    index+=1


# In[21]:


import subprocess
cp = subprocess.run("Singular<SCRIPT.txt", shell=True,capture_output=True,text=True)
print("stdout:", cp.stdout)
print("stderr:", cp.stderr)


# In[5]:


import numpy as np
import csv
def getmat(filename):
    rowmx=list()
    with open(filename, 'r') as file:
        reader = csv.reader(file)
        for t in reader:
            #print(t)
            rowmx.append(t)
    x=rowmx[0]
    y=np.array([eval(t) for t in x])
    return np.array(np.array_split(y,8))

mx=getmat('save_mx.txt')    
my=getmat('save_my.txt')    
me=getmat('save_me.txt')    


# In[7]:


ee


# In[ ]:


ee,vv=np.linalg.eig(mx)
ww=vv.transpose()
ee


# In[ ]:


ee,vv=np.linalg.eig(mx)
ww=vv.transpose()
for eee,www in zip(ee,ww):
    if np.abs(np.imag(eee)) < 1.0e-10:
        #print(eee)
        print([np.real(np.dot(www.conj(),np.dot(mop,www))) for mop in [mx,my,me]])


# In[ ]:


np.linalg.eig(my)


# In[ ]:


str(ENT.expand())


# In[ ]:


getF.subs(R,1.407)


# In[ ]:


for i in range(2):
    for j in range(2):
        for k in range(2):
            for l in range(2):
                print(TT[i][j][k][l].subs(R,1.46))


# In[ ]:


1.30715160755548
0.437279325265417
0.437279325265417
0.605703366333600
0.437279325265417
0.177267121950662
0.177267121950662
0.311794570368974
0.437279325265417
0.177267121950662
0.177267121950662
0.311794570368974
0.605703366333600
0.311794570368974
0.311794570368974
0.774608360032879


# In[ ]:


-5.20404549877700
-1.34720517231307
-1.34720517231307
-2.48776936801926


# In[ ]:


[[1.00000142599786, 0.450770411647788], [0.450770411647788, 1.00000142599786]]
[[2.16431256194901, 0.167012865864049], [0.167012865864049, 0.760032943565085]]
KAB
KAB


# In[ ]:


for i in range(2):
    for j in range(2):
        if i!=j:
            print(S[i][j].subs(R,1.46))
        else:
            print(S[i][j])


# In[ ]:


T12.subs(R,1.46)


# In[ ]:


for i in range(2):
    for j in range(2):
                print(H[i][j].subs(R,1.46))


# In[ ]:


[V11A,V12A,V22A,V11B,V12B,V22B]


# In[ ]:


for x in [V11A,V12A,V22A,V11B,V12B,V22B]:
    print(x.subs(R,1.46))


# In[ ]:


V11A.subs(R,1.46)


# In[ ]:


for i in range(2):
    for j in range(2):
        for k in range(2):
            for l in range(2):
                print(TT[i][j][k][l].subs(R,1.46))


# In[ ]:


V2211.subs(R,1.46)


# In[ ]:


OF=getF-2*e*getNS
OF.subs(R,1.46).expand()


